We Think, Therefore We Align LLMs to Helpful, Harmless and Honest Before They Go Wrong

Alignment of Large Language Models (LLMs) is the ability to satisfy desired objectives during generation, which is critical for trustworthy deployment. In practice, alignment is often operationalized through multiple objectives such as Helpfulness, Harmlessness, and Honesty (HHH). Prior works study alignment via steering vectors in standard Transformer decoders but treat objectives in isolation, where optimizing a single objective can overwrite others, leading to interference. Recent works attempt to address this limitation by extending steering to a 1-to-N Transformer setting by replicating representations into objective-specific pathways, but apply transformations independently, resulting in inconsistent responses across objectives. Similarly, approaches such as safe RLHF and MoE-based designs study trade-offs across objectives but do not constrain objective-specific transformations within a shared representation during inference. As a result, even aligned State-of-the-Art (SOTA) LLMs can struggle to jointly satisfy HHH objectives in complex settings. To address this, we propose Adaptive Multi-Branch Steering (AMBS), a two-stage framework in a 1-to-N Transformer setting that parameterizes objective-specific transformations relative to a shared representation. In Stage I, a shared hidden representation is computed once. In Stage II, this representation is replicated into N pathways and updated relative to a shared reference, capturing objective-specific deviations while restricting divergence. This produces N objective-specific responses within a single forward pass, which can be combined at decoding to obtain a single response across objectives. Across multiple backbones, AMBS improves performance across HHH, with consistent gains in WR, TI, and SS (e.g., Avg 56.5% on LLaMA-2-7B) while maintaining efficiency (e.g., 189 Tok/s, 9 GPU-hrs).

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction (see \S\ref{Introduction}) clearly state the core contribution—Adaptive Multi-Branch Steering (AMBS) for multi-objective alignment—and claim improved joint HHH performance with reduced interference, which is directly supported by experimental results in \S\ref{Result and Analysis} and ablation studies in \S\ref{Ablation Study}.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper discusses limitations in \S\ref{Conclusion}, including limited human evaluation scale, reliance on proxy automatic judges, and restriction to decoder-only models, along with directions for future work.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper includes formal statements (Lemmas 1–3) (see \S\ref{Shared Steering}) with clearly defined assumptions and complete empirical proofs provided in \S\ref{Ablation Study}.

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper provides detailed descriptions of the AMBS framework, including equations (Eqs. 2–10) (see \S\ref{Methodology}), dataset usage and splits (see \S\ref{Dataset}), model backbones (see \S\ref{Baselines}), and hyperparameters (see \S\ref{Hyperparameters}), which together are sufficient to reproduce the experimental setup and results.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper provides anonymized code in the supplementary material along with references to publicly available datasets and pretrained models, for reproduction of the main experimental results.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: \S\ref{Experimental Setup} specifies datasets and splits (see \S\ref{Dataset}), model architectures (see \S\ref{Baselines}), hyperparameters (see \S\ref{Hyperparameters}), and evaluation metrics (see \S\ref{Evaluation Metrics}), for a clear understanding of the experimental setup.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: The paper reports average performance metrics and includes limited variance analysis across three random seeds (see \S\ref{Ablation Study}), but does not provide formal error bars, confidence intervals, or statistical significance tests for the main results.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: \S\ref{Hyperparameters} specifies the compute setup, including training on a single NVIDIA A100 (80GB), training duration (GPU-hours), throughput (tokens/s), and memory usage, which together provide sufficient detail to estimate computational requirements (see \S\ref{Result and Analysis}).

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The research uses publicly available datasets (see \S\ref{Dataset}) and pretrained models (see \S\ref{Baselines}), does not involve human subjects or sensitive personal data, which is consistent with the NeurIPS Code of Ethics.


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper focuses on improving alignment along helpfulness, harmlessness, and honesty, it does discuss broader societal impacts, including potential risks such as misuse or unintended consequences in \S\ref{Introduction}.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not release new datasets or pretrained models, and instead builds on existing publicly available datasets (see \S\ref{Dataset}) and pretrained models (see \S\ref{Baselines}); therefore, no additional safeguards are required for release.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper cites and references publicly publicly available datasets (see \S\ref{Dataset}) and pretrained models (see \S\ref{Baselines}), but does not state the licenses or terms of use for these assets within the paper.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not introduce new datasets, pretrained models, or standalone assets, and instead builds on existing publicly publicly available datasets (see \S\ref{Dataset}) and pretrained models (see \S\ref{Baselines}).

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper includes a small-scale human evaluation (150 instances annotated by three graduate-level NLP researchers) but does not involve crowdsourcing or provide detailed annotation protocols, instructions, or compensation information, as this evaluation is used only for qualitative validation rather than as a primary experimental component (see \S\ref{Ablation Study}).

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve formal human subjects research or data collection. The limited human evaluation is conducted on existing model outputs without sensitive data or interaction with external participants, and does not constitute a study requiring IRB approval.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research?
    \item[] Answer: \answerYes{}
    \item[] Justification: LLM-based evaluators are used for assessing HHH, which are described in \S\ref{Dataset}.

\end{enumerate}
